A Novel Approach to Finding Near-Cliques: The Triangle-Densest Subgraph Problem

Many graph mining applications rely on detecting subgraphs which are near-cliques. There exists a dichotomy between the results in the existing work related to this problem: on the one hand the densest subgraph problem (DSP) which maximizes the average degree over all subgraphs is solvable in polynomial time but for many networks fails to find subgraphs which are near-cliques. On the other hand, formulations that are geared towards finding near-cliques are NP-hard and frequently inapproximable due to connections with the Maximum Clique problem. In this work, we propose a formulation which combines the best of both worlds: it is solvable in polynomial time and finds near-cliques when the DSP fails. Surprisingly, our formulation is a simple variation of the DSP. Specifically, we define the triangle densest subgraph problem (TDSP): given $G(V,E)$, find a subset of vertices $S^*$ such that $\tau(S^*)=\max_{S \subseteq V} \frac{t(S)}{|S|}$, where $t(S)$ is the number of triangles induced by the set $S$. We provide various exact and approximation algorithms which the solve the TDSP efficiently. Furthermore, we show how our algorithms adapt to the more general problem of maximizing the $k$-clique average density. Finally, we provide empirical evidence that the TDSP should be used whenever the output of the DSP fails to output a near-clique.

==> Streaming.tex <==
Our analysis in the previous sections indicates the importance 
of creating a good initial seed. We propose a system which produces fast,
high-quality results based on the ideas presented in Section~\ref{sec:proposed}. 
On the one hand, it is clear from existing work \cite{fennel, stantonkliot}
that degree-based heuristics can improve significantly the quality of default graph 
parirtitioners in many graph-processing systems such as \reminder{Giraph etc}.
As our analysis shows, the performance of \cite{fennel, stantonkliot} can be further 
improved in terms of the running time by using for a high degree vertex $v$ 
a polylogarithmic number  of its neighbors in order to estimate 
the number of neighbors it has in each of the clusters. 
On the other hand, our analysis  which complements Stanton's recent work \cite{} 
strongly indicates that these heuristics can be further enhanced when  
we allow a small computational overhead for the first steps of the process in order 
to create a good initial seed. 
Such an overhead could be by using an existing partitioning tool such as METIS \cite{},
McSherry's spectral algorithm \cite{} or the simple 2-path classification criterion
of Section~\ref{subsec:path2classification}. 
Our proposed system \Egypt is a streaming algorithm that applies these two ideas. 
It firsts creates a 


the partitioning 
processis initialized with a good seed. 

On the other hand, a small computational overhead in the beginning of the process 
can significantly improve 


While one can come up wiy

For practical purposes we propose combining the ideas 
to 


We derive a streaming algorithm by using a greedy assignment of vertices to clusters as follows: assign each arriving vertex to a partition such that 
the objective function of the $k$ graph partitioning problem, defined as a maximization problem, is increased the most. 
Formally, given that current vertex partition is $\mathcal{P} = (S_1,S_2,\ldots,S_k)$, a vertex $v$ is assigned to partition $i$ such that
\begin{eqnarray*}
&& g(S_1,\ldots,S_i\cup \{v\},\ldots,S_j,\ldots,S_k)\\
&\geq & g(S_1,\ldots,S_i,\ldots,S_j\cup \{v\},\ldots,S_k), \hbox{ for all } j\in [k].
\end{eqnarray*}  
Defining $\delta g(v,S_i) = g(S_1,\ldots,S_i\cup \{v\},\ldots,S_j,\ldots,S_k) - g(S_1,\ldots,S_i,\ldots,S_j,\ldots,S_k)$, the above greedy vertex assignment
naturally suggests the following streaming algorithm. 

\begin{center}\fbox{
\begin{minipage}{0.8\linewidth}
\textbf{Greedy vertex assignment}
\begin{itemize}
    \item Assign vertex $v$ to partition $i$ such that $\delta g(v,S_i) \geq \delta g(v,S_j)$, for all $j\in [k]$\\
\end{itemize}
\end{minipage}
}
\end{center}

Finally, we outline that in many applications there exist very strict constraints 
on the load balance. Despite the fact that we investigate the effect of the parameter 
$\gamma$ on the load balance, one may apply the following algorithm, which enforces 
to consider only machines whose load is at most $\nu \times  \frac{n}{k}$.
This algorithm for $1 \leq \gamma \leq 2$ amounts to interpolating between 
the basic heuristics of \cite{stanton} and \cite{Prabhakaran:2012:MLG:2342821.2342825}.
The overall complexity of our algorithm is $O(n+m)$. 


\begin{center}\fbox{
\begin{minipage}{0.85\linewidth}
\textbf{Greedy vertex assignment with threshold $\nu$}
\begin{itemize}
    \item Let $I_{\nu}=\{i: \mu_i \leq \nu \frac{n}{k} \}$. 
    Assign vertex $v$ to partition $i\in I_\nu$ such that $\delta g(v,S_i) \geq \delta g(v,S_j)$, for all $j\in I_\nu$
    
%	Assign vertex $v$ to partition $i \in I_{\nu}$ such that 
%	$|N(v) \cap S_i| - \delta c(|S_i|) \geq |N(v) \cap S_j| - \delta c(|S_j|)$, for all $j \neq i, j \in I_{\nu}$. 
\end{itemize}
\end{minipage}
}
\end{center}


\medskip
\label{alg:alg3}
\framebox{
\begin{minipage}[b]{1\linewidth}
\begin{enumerate} 
%\item Place the inter- and intra-cluster edges in the correct machines. 
\item For the $j$-th edge $e_j=\{u,v\}$, $j \geq f(n)+1$ 
	\begin{itemize}
               \item Sample randomly $C\log^{1+\gamma}(n)$ vertices from each machine, where $\gamma>0$ is a constant. 
		Let $\Gamma_j$ be the resulting sample. 
		\item Compute  in how many triangles edge $\{u,v\}$ participates, let it be $X$. 
	       \item  Fix some $\delta>0$. If  $ X \geq (1-\delta) (p^2+(k-1)q^2) |\Gamma_j|$ then 
              $\Psi(u)=\Psi(v)$. If not place it in the other machine. In the former case, sample again to find 
             the correct machine.
	\end{itemize} 
\end{enumerate} 
\end{minipage}
\medskip\par}
